How Trans-Inclusive are Hackathons?

Hackathons are fun! People go there to learn, meet new colleagues, intensively work on a collaborative project, and mix pizza with energy drinks. However, for transgender community and other minorities, hackathons can have an uncomfortable atmosphere. Some transgender and non-conforming people that, although enjoying hackathons, decided not to participate anymore, afraid of LGBQTPhobia and other discomforts. In this paper we surveyed 44 trans and cis hackathons participants and interviewed seven transgender ones. By understanding their needs and challenges, we introduce five recommendations to make hackathons more inclusive.

==> links.tex <==
Cronograma e códigos: https://docs.google.com/spreadsheets/d/1K7nwkixXNvFiQPipISN3D0rIp8BrYshTeAktuYnJsaA/edit?usp=sharing

Pasta com entrevistas e referências:
https://drive.google.com/drive/folders/1r6Mun9qM_2Dq5tHKaLbYSYxDMegm9zRh?usp=sharing

form:
https://docs.google.com/forms/d/1b31SGq4HGfUBsJuCcaYTzp_e-vOT9Sv0rVb_b3zmEMM/edit?usp=sharing

Respostas do form:
https://docs.google.com/spreadsheets/d/1l-0ElcJceawZKMaa3qDy8v03inLNQFqmhPjxxmpocP8/edit?usp=sharing
